Trained Without My Consent: Detecting Code Inclusion In Language Models Trained on Code

Code auditing ensures that the developed code adheres to standards, regulations, and copyright protection by verifying that it does not contain code from protected sources. The recent advent of Large Language Models (LLMs) as coding assistants in the software development process poses new challenges for code auditing. The dataset for training these models is mainly collected from publicly available sources. This raises the issue of intellectual property infringement as developers' codes are already included in the dataset. Therefore, auditing code developed using LLMs is challenging, as it is difficult to reliably assert if an LLM used during development has been trained on specific copyrighted codes, given that we do not have access to the training datasets of these models. Given the non-disclosure of the training datasets, traditional approaches such as code clone detection are insufficient for asserting copyright infringement. To address this challenge, we propose a new approach, TraWiC; a model-agnostic and interpretable method based on membership inference for detecting code inclusion in an LLM's training dataset. We extract syntactic and semantic identifiers unique to each program to train a classifier for detecting code inclusion. In our experiments, we observe that TraWiC is capable of detecting 83.87% of codes that were used to train an LLM. In comparison, the prevalent clone detection tool NiCad is only capable of detecting 47.64%. In addition to its remarkable performance, TraWiC has low resource overhead in contrast to pair-wise clone detection that is conducted during the auditing process of tools like CodeWhisperer reference tracker, across thousands of code snippets.

==> Sections/methodology.tex <==
In this section, we present the methodology that we followed for our approach as displayed in Figure \ref{fig:methodology_overview}. As explained in \ref{subsec:background__mia}, memorization can be leveraged in MIAs in order to investigate the presence of data records in a model's training dataset. Previous works have used \textit{exact memorization} \cite{tirumala2022memorization} and \textit{name cloze} \cite{chang2023speak} approaches to analyze the outputs of a model for detecting data inclusion. In both works, parts of the input to the model are \textbf{masked}, and the model is tasked with predicting the masked element given the rest of the input as context. Finally, the model's outputs are inspected in order to look for tokens that the model should not be able to predict correctly unless it has seen them during its training. In our work, we follow the same rationale with some modifications with respect to code. We consider code as consisting of two distinct parts: \textbf{syntax} and \textbf{documentation}; with syntax being the code itself (which follows the programming language's structural rules) and documentation being an explanation of the syntax for future reference. From here on, we use the word \textit{``script''} to denote a single file in a project that contains the code alongside its documentation. We formally define masking as follows:

\begin{center}
    \textbf{Definition 1: }\textit{Given input $I$ which consists of tokens $[t_1, t_2, ..., t_n]$, and a chosen token $T$, masking $T$ entails replacing all the tokens in $I$ which match $T$ with another token named $MASKED$. The model $M$ is queried to predict what $MASKED$ is, given the $I$ as input.}
\end{center}

We also define exact and partial matching of masked elements as follows:

\begin{center}
    \textbf{Definition 2: }\textit{Let $I$ be an input composed of a sequence of tokens $[t_1, t_2, ..., t_n]$ with a specific token $T$ masked. An \underline{exact match} is detected if the output of model $M$ for the masked token $T$ is identical to the actual token $T$.}
\end{center}

\begin{center}
    \textbf{Definition 3: }\textit{Let $I$ be an input composed of a sequence of tokens $[t_1, t_2, ..., t_n]$ with a specific token $T$ masked. Given a similarity function $S$, a \underline{partial match} is detected if the similarity score $S(M(I), T)$ produced by model $M$ for the masked token $T$ surpasses a specified threshold $L$.}
\end{center}

In alignment with established coding standards, such as those described in \cite{martin2009clean}, it is essential that variable/function/class names be selected in a manner that reflects their purpose and context within the codebase. These identifiers, beyond the common ones that are universally used, are unique to the script and its corresponding project and reflect the developers' personal coding style. Additionally, documentation, which is an important part of coding, is closer to natural language as it is not constrained to the programming language's syntax and therefore, allows for a greater expression of the developers' individual styles \cite{ying2005source, fluri2007code}. Therefore, in order to detect whether a project (collection of scripts) was used in a model's training dataset, we break each script into 2 different identifier groups and compare the model's generations with the inputs as follows:

\begin{itemize}
    \item \textbf{Syntactic identifiers}: As these identifiers are unique to the codebase, we look for exact matches between the masked elements in the original script and the model's outputs:
        \begin{enumerate}
            \item Variable names
            \item Function names
            \item Class names
        \end{enumerate}
        
    \item \textbf{Semantic identifiers}: As these identifiers are closer to natural language than code, we look for partial matches between the masked elements and the model's outputs:
        \begin{enumerate}
        \setcounter{enumi}{3}
            \item Strings (data structures that are used to handle textual data) \Foutse{only textual data??? why? are you suggesting that the generated programs only manipulate textual data??? or is it something else} \ahura {no. I mean the literal string data type}
            \item Comments (explanation of a piece of code's functionality)
            \item Docstrings (explanations of a function's or class's functionality). It should be noted that we categorize docstrings in a different group than comments regardless of the programming language. We consider DocStrings to be parts of the documentation that specifically describe a function/class's functionality. These elements are usually longer and rarer than comments. \Foutse{this is Python specific !!! in other programing languages comments are used...hence my second question, how is it different from your comment category above???} \ahrua{I'm setting a difference between comments that are not describing an entire function and class's  functionality and those that do. docstrings are normally much longer than comments and rarer. therefore they need their own category}
        \end{enumerate}
\end{itemize}

 We aim to identify whether a project (which may consist of multiple scripts) was included in an LLM's training set.
To do so, we break each script into 6 different elements:
    


For syntactic identifiers, if the model generates an incorrect \Foutse{then the incorrect here is with respect to the context of the program under development and not incorrect with respect to training data...please check your previous definition since your notion of 'original script' there seems not to reflect what you are explaining here!} output (whether incorrect variable/function/class names or incorrect syntax such as incorrect operations), the generated code will not run/compile. However, such a problem does not exist for the \Foutse{also, calling comments 'semantic identifiers' is ambiguous since semantic identifiers already have a dedicated meaning!!!}semantic identifiers of the script. These elements are an explanation of how the code is supposed to work and are written in natural language (as opposed to pure code). If the model generates an incorrect explanation, the code will continue to function without generating any errors.

In our approach, we first extract the syntactic and semantic identifiers from the original script by parsing the code. Afterward, each extracted element is masked and the model is queried to predict the masked element. We define \textit{masking} as omitting the extracted element from the rest of the script. After collecting the model's outputs, \Foutse{we have not provided a good intuition as to why correctly predicting these masked elements would be a sign of memorization...what is very unique in them? that has not been demonstrated so far...it sounds like we randomly tried masking certain thing and that happened to work} we look for the degree of similarity between the generated outputs and the original masked elements to determine whether the script was included in the model's training dataset. It should be noted that we mask only the extracted element and leave the rest of the script as it originally was. 
% We theorize that by inputting queries that are the same as what the model was trained on, the model will output what is similar to its training data. 
Figure \ref{fig:methodology_overview} displays our overall approach which consists of four stages: pre-processing, inference, comparison, and classification which we explain in detail in the following.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Pictures/methodology_overview.png}
    \caption{Methodology Overview}
    \label{fig:methodology_overview}
\end{figure}


\subsection{Decision Making Pipeline}\label{subsec:methodology__decision_making_pipeline}
    \subsubsection{Pre-processing}\label{subsec:methodology__preprocessing}
        As stated, we break each script into its six constituent elements (i.e. syntactic/semantic identifiers). From each script, we extract the elements and for each extracted element, we break down the code into two parts: A part that comes immediately before the extracted element (prefix) and the part that comes after the extracted element (suffix). For example, Listings \ref{listing:example_function_prefix} and \ref{listing:example_function_suffix} display the prefix and suffix generated for the function outlined in Listing \ref{listing:example_function_whole_code} for the variable \underline{\texttt{string\_to\_print}}. By creating a prefix and suffix pair for each extracted element, we will be able to query the model to generate what comes in between which we will explain in the rest of this section.
        
        \noindent\begin{minipage}{\textwidth}
            \begin{minted}[bgcolor=lightgray]{python}
                def print_string():
                    string_to_print = "Hello World!"
                    print(string_to_print)
            \end{minted}
            \captionof{listing}{A function in a script}
            \label{listing:example_function_whole_code}
        \end{minipage}
        
        
        \noindent\begin{minipage}{\textwidth}
            \begin{minted}[bgcolor=lightgray]{python}
                def print_string():
            \end{minted}
            \captionof{listing}{Prefix}
            \label{listing:example_function_prefix}
        \end{minipage}
        
        
        \noindent\begin{minipage}{\textwidth}
            \begin{minted}[bgcolor=lightgray]{python}
                                        = "Hello World!"
                    print(string_to_print)
            \end{minted}
            \captionof{listing}{Suffix}
            \label{listing:example_function_suffix}
        \end{minipage}

    \subsubsection{Inference}\label{subsec:methodology__inference}
        One of the techniques that is used in both pre-training and fine-tuning of LLMs is partially masking the input and having the model generate the masked part \cite{bavarian2022efficient}. This is referred to as \textit{Fill-In-the-Middle} (FIM) in which the original text is broken into three parts: prefix, masked element, and suffix. The model is then tasked to predict the masked element given the prefix and suffix as input. For our approach, we follow the same approach. The aim of breaking each script into multiple (prefix, suffix) tuples is to leverage the problem of memorization in LLMs. More specifically and as mentioned in Section \ref{subsec:background__copyright_in_ml}, as the capacity (i.e. number of parameters) of ML models increases, so does their ability to memorize their training dataset instead of generalizing (i.e. learning). Therefore, by using a large part of the script that was present in the model's training dataset as input, and only masking a small piece (i.e., a single element), the model would be pushed in the direction of generating an output that is the same or highly similar to what was present in its training dataset. Once we have collected all the model's outputs for the extracted elements for a script, we move to the next step in which we compare the model's outputs with the original elements.
        
    \subsubsection{Comparison}\label{subsec:methdology__comparison}
        Given the outputs of the model for each element, we define two different comparison criteria given the element's type:
            \begin{itemize}
                \item For syntactic identifiers (Variable/Function/Class names), we look for an \textbf{exact} match. If the model generates the exact same token(s), we count it as a \textit{“hit”}, which is a binary flag that indicates whether the generated output matches the desired output.
                
                \item For semantic identifiers (strings/documentation), to assess the similarity between two sequences (series of tokens), we use the Levenshtein distance (edit distance) score \cite{levenshtein_distance}. This metric measures the number of single-character edits that are required to change one sequence to the other. These elements are closer to natural language and do not require the syntactic restrictions required for code (incorrect/inaccurate generations will not result in syntax errors). Therefore, we compare the generated output with the original tokens and calculate the edit distance between the two. Here, we define a threshold, and edit distances higher than this threshold will be considered as a \textit{hit}. The final threshold was chosen empirically to provide a balance between semantic similarity and performance gains. We present the results with different thresholds in Section \ref{sec:results}.
                
                The other metrics that can be used for this objective are based on semantic similarity where a semantic score is calculated between the vector representations of two strings (e.g. cosine similarity, TF-IDF distance, etc.) \cite{wang2020measurement}. We choose the edit distance metric as we do not aim to inspect whether the model's output is similar to the original masked element in meaning but in syntactic structure. Therefore, analyzing the semantic distance would not be helpful for this task.
            \end{itemize}
        
        After processing the model's outputs as described above, we normalize the hit numbers by dividing the number of hits against the total number of checks for each type of identifier. Table \ref{table:ds_sample} shows a sample of the dataset that is constructed for inclusion detection.
                
        \begin{table}
            \centering
            \caption{Data Representation Sample}
            \begin{adjustbox}{max width=\textwidth}
                \begin{tabular}{lrrrrrr}
                \toprule
                Script Name & Class Hits & Function Hits & Variable Hits & String Similarity & Comment Similarity & Docstring Similarity \\
                \midrule
                zhongchun/mars/tokenize.py & 0.33 & 1.0 & 0.08 & 0.4 & 0.66 & 0.0 \\
                0mars/mailgun-sdk/base.py & 0.6 & 0.46 & 0.5 & 0.04 & 0.0 & 0.22 \\
                \bottomrule
                \end{tabular}
            \end{adjustbox}
            
            \label{table:ds_sample}
        \end{table}

    \subsubsection{Classification}
        % After the datasets for inclusion detection are constructed, our task becomes a binary classification problem. \Amin{from the beginning it is a classification task, no?}
        With our extracted tractable features, the classifier's task is to detect whether a script was included in the LLM's training dataset; which makes this a binary classification problem. Any classification method, such as decision trees or Deep Neural Networks (DNN), can be used based on the desired performance. 

\subsection{Comparison With Clone Detection Approaches}\label{subsec:methodology__comparison_with_nicad}
    In software auditing, one of the approaches for detecting copyright infringement is using CCDs to check the code against a repository of copyrighted code \cite{ralhan2021study}. CCD is an active area of research and different approaches are proposed for the detection of clones, especially those of \textit{Type 3} and \textit{Type 4} \cite{ain2019systematic}. This process is carried out through a pair-wise comparison of the codes in a project against another dataset that contains copyrighted codes. As detailed in Section \ref{subsec:background__code_clone_detection}, many different approaches are proposed and available for CCD \cite{ain2019systematic}. Out of the proposed approaches, we choose NiCad \cite{roy2008nicad} to compare TraWiC with on the code inclusion task for the following reasons:

    \begin{itemize}
        \item \textbf{Python support:} Out of the tools that are presented, NiCad is the only one that supports clone detection for Python scripts.
        \item \textbf{Availability:} A few of the proposed approaches are available for use. Furthermore, most of them require expensive re-training on new datasets. However, NiCad is open-source and does not require re-training (as opposed to the proposed DL-based solutions).
        \item \textbf{Syntactic errors in generated codes:} Most of the proposed approaches for CCD based on DNNs, extract information such as ASTs from the code which can only be done if the generated code is syntactically valid. Even though LLMs have shown a high capability in generating correct code, limiting CCD to codes that are syntactically valid would severely reduce the size of the dataset that can be used for this purpose.
    \end{itemize}

    NiCad employs a parser-based, language-specific approach using the TXL transformation system to extract and normalize potential code clones. As NiCad is designed to detect clones between scripts, it operates differently compared to our approach where we inspect the similarity between one or multiple generated tokens. Therefore, to determine whether a code was in a model's training dataset with NiCad, we query the model to generate code snippets and compare the generated codes against each snippet that we know exists in the model's training dataset. We generate code snippets instead of tokens since comparing scripts to each other using NiCad will result in positive clone matches as a large portion of both codes will be the same. Our detailed process is as follows:

    \subsubsection{Pre-processing}\label{subsubsec:methodology__nicad__preprocessing}
        We extract the functions and classes that are defined in a script by parsing its code. After doing so, we break each function/class into two parts based on its number of lines. Listings \ref{listing:nicad_example_function_whole_code}, \ref{listing:nicad_example_function_prefix}, and \ref{listing:nicad_example_function_suffix} display an example of how this process is carried out. This process is repeated for every function and class that is extracted from the script. We consider the first half as the prefix and the second half as the suffix.
        
            \noindent\begin{minipage}{\textwidth}
                \begin{minted}[bgcolor=lightgray]{python}
                def calculate_average(list_of_numbers):
                    sum_of_elements = 0
                    for i in list_of_numbers:
                        sum_of_elements = i + sum_of_elements
                    average = sum_of_elements / len(list_of_numbers)
                    return average
                \end{minted}
                \captionof{listing}{A function extracted from a script}
                \label{listing:nicad_example_function_whole_code}
            \end{minipage}
            
            
            \noindent\begin{minipage}{\textwidth}
                \begin{minted}[bgcolor=lightgray]{python}
                def calculate_average(list_of_numbers):
                    sum_of_elements = 0
                    for i in list_of_numbers:  
                \end{minted}
                \captionof{listing}{The first half of the script (by the number of lines)}
                \label{listing:nicad_example_function_prefix}
            \end{minipage}
            
            
            \noindent\begin{minipage}{\textwidth}
                \begin{minted}[bgcolor=lightgray]{python}
                    sum_of_elements = i + sum_of_elements
                    average = sum_of_elements / len(list_of_numbers)
                    return average
                \end{minted}
                \captionof{listing}{The second half of the script (by the number of lines)}
                \label{listing:nicad_example_function_suffix}
            \end{minipage}


    \subsubsection{Inference}\label{subsubsec:methodology__nicad__inference}
        After generating prefix and suffix pairs, we query the model with the prefix and have the model generate the suffix. Note that here, we do not restrict the model to predict the masked element by giving it the suffix. Instead, we allow the model to generate what comes after the prefix until the model itself generates an ``end-of-sequence'' token.

    \subsubsection{Comparison}\label{subsubsec:methodology__nicad__comparison}
         % Given the size of TheStack dataset (106.91 million Python scripts), comparing each generated script in a pair-wise manner against all the other scripts present in the training dataset is computationally infeasible. Therefore, we first consider a minimum and maximum number of scripts per repository as a sampling criteria. We consider a project for sampling if it contains more than 10 and less than 50 scripts. By doing so we increase the chances that a project was included in the model's training set. After doing so, we sample entire projects in a random manner from the resulting dataset.
         We compare each generated script with those of multiple randomly sampled repositories from the model's training dataset to detect code clones across projects. Here, our aim is to investigate whether the model generates codes from its training dataset when it is given a large part of a script as input. If NiCad detects a clone between the generated script and another script from the sampled projects, we consider it as a \textit{hit} for detecting that the project was included in the model's training dataset. NiCad is capable of detecting code clones up to Type 3 \cite{roy2008nicad}.

==> dump.tex <==
% ####### OLD RELATED WORKS 
    % \section{Related Works}\label{sec:related_wors}
    %     As mentioned in Section \ref{subsec:background__copyright_in_ml}, most research in the ML community is focused on watermarking the outputs of an ML model. However, advances in GenAI have resulted in the researchers devising methods for identifying the dataset of an ML model without access to the dataset itself. Attempts at reconstructing the training dataset by querying the model are referred to as Membership Inference Attacks (MIA). Shokri et al. \cite{shokri2017membership} studied how an attacker can identify the presence of a record in a model's training dataset by analyzing the model's output probabilities. Based on Shokri et al.'s work, many approaches have been proposed for both attacks on a model for extracting information about its training dataset and defenses in order to prevent the model from recreating sensitive records \cite{shokri2017membership, jia2019memguard, hu2021ear, hui2021practical}. Carlini et al. \cite{carlini2021extracting} attempted to extract the training data of GPT-2 by initializing the model with a sequence start token and having the model generate tokens until it generates an end-of-sequence token. They generate a large number of sequences in this fashion and remove samples that contain low likelihood. Their approach is based on the idea that samples with high likelihood are generated either because of trivial memorization or repeated sub-strings in their dataset. By doing so, they were able to extract information about individuals' contact information, news pieces, tweets, etc. In another work, Carlini et al. \cite{carlini2022quantifying} study the quantity of memorization in LLMs. They show that by increasing the number of parameters of a model, the amount of memorized data increases as well. Chang et al. \cite{chang2023speak} attempt to probe ChatGPT and GPT-4 by using ``name cloze'' membership inference queries. In their approach, they query ChatGPT/GPT-4 by giving it a context (which in their work are texts extracted from novels), mask the token which contains a \textit{name}, and inspect the output's similarity to the original token. The underlying idea is that without the model seeing the input during its training, the name should be impossible to predict. ``Counterfactual Memorization'' \cite{zhang2021counterfactual} is another approach proposed for studying the memorization issue in LLMs. Here, the changes in a model's predictions are characterized by omitting a particular document during its training. Even though this approach shows promise in studying a model's degree of memorization, it is very computationally expensive. To the best of our knowledge, there exists no approach that inspects \textit{LLMs trained on code} in order to detect data inclusion.

% ####### OLD BACKGROUND
   % In this section, we review the subjects that are required for understanding our work. Specifically, our methodology is tailored for use with LLMs trained on code, therefore, we will review the background and the necessary concepts in this area.
    % % In this section, we will review the related works \Foutse{is this a related work section or a background section???} and subjects to our approach. Our approach is designed to work with LLMs trained on code, therefore, we will review the background and the necessary concepts in this area. 
    % Afterward, we will go over code clone detection as they can be used for code inclusion detection in datasets of LLMs (albeit with high compute costs). Finally, we will briefly review the current works and discussions about detecting ML-generated content.
    
    % \subsection{Large Language Models}\label{subsec:background__llms}
    %     One of the highly active fields of research in ML is Natural Language Processing (NLP). Here, research is focused on designing approaches that are capable of understanding language and generating responses that are contextually relevant, accurate, and coherent.
    %     % \Foutse{you are missing a sentence giving the context in which these studies occurred and why they occurred this way!!!} 
    %     Neural Language Models (NLMs) were trained in order to predict the probability of the next word (token) in a sequence by considering the previous tokens \cite{qiu2020pre}. Models such as ELMo \cite{peters2018deep} and BERT \cite{devlin2018bert} were introduced by training a model on a large dataset of unlabeled corpora to learn word representations based on the context (other tokens in the sequence). This process is known as \textit{pre-training}; a model is trained on an unlabeled dataset to learn word representations, language structure, syntax, and semantics \cite{petroni2019language, feldman2019commonsense}. Pre-trained models can be further \textit{fine-tuned} for specific tasks by continuing their training on a labeled dataset designed for the task at hand. By incorporating the Transformer architecture and using the self-attention mechanism \cite{vaswani2023attention}, models such as GPT-2 \cite{radford2019language} were trained using the pre-training/fine-tuning paradigm alongside introducing new architectures. Models such as GPT-3 \cite{brown2020language} were trained by mainly using similar architectures but scaling the size of the model alongside its training data. As the number of these models' parameters is extremely large, they are called \textit{Large Language Models}. Code is even used in the training dataset of LLMs that are not fine-tuned for program synthesis as it has been shown to increase a model's capability in reasoning \cite{chen2021evaluating, austin2021program}. LLMs have displayed high performance in coding tasks from easy to complex by being fine-tuned on large datasets of code. Currently, enterprises are offering LLMs fine-tuned for coding tasks such as GitHub's Copilot (based on Codex \cite{chen2021evaluating}), Amazon's CodeWhisperer, and Google's Codey. Alongside these enterprise services, many open-source models such as SantaCoder \cite{allal2023santacoder}, WizardCoder \cite{luo2023wizardcoder}, CodeLlama \cite{rozière2023code}, etc., are available. These LLMs were trained using different approaches, are based on various architectures, and are designed to achieve different objectives (program synthesis, code summarization, comment generation, etc.). However, regardless of their intended use, all of these models require a large corpus of high-quality code (code that contains documentation explaining the functionality of its different parts) during their pre-training and fine-tuning phases. The primary resources for collecting such data are GitHub and StackOverflow, which contain vast amounts of open-source codes, and most of the open-source datasets online (e.g. TheStack \cite{Kocetkov2022TheStack}) are just an accumulation of data collected from these resources.  
        
    % \subsection{Code Clone Detection}\label{subsec:background__code_clone_detection}
    %     Code Clone Detection (CCD) is a widely researched area and is an important aspect of assessing software quality. A fault/bug/vulnerability that is present in one project can exist in other projects that contain similar codes and correction is required for all clones. Other software engineering activities such as plagiarism detection, program understanding, code compaction, etc. require identifying codes that are similar to each other either semantically or syntactically as well \cite{roy2009comparison}. CCD tools such as NiCad \cite{roy2008nicad}, SorcererCC \cite{sajnani2016sourcerercc}, Simian \cite{simian_ccd}, etc., are available as either open-source or enterprise tools to facilitate CCD activities. In CCD literature, code clones are categorized into four categories \cite{roy2007survey}: 
        
    %     \begin{itemize}
    %         \item \textit{Type-1:} An exact copy without modifications (except for whitespace and comments).
    %         \item \textit{Type-2:} A syntactically identical copy with differences in variable/type/function identifiers.
    %         \item \textit{Type-3:} Similar code fragments with extra addition or deletion of statements.
    %         \item \textit{Type-4:} Code fragments with different syntax, but similar semantics. 
    %     \end{itemize}
        
    %     By exploiting the powerful representation learning ability of Deep Learning (DL), a large amount of research has been conducted on using DL-based approaches for CCD. To detect clones, these models use various code representations such as Abstract Syntax Trees (AST), Control Flow Graphs (CFG), code metrics (number of functions, number of variable calls, etc.), and raw code itself. DL-based approaches such as CoCoNut \cite{lutellier2020coconut}, AST-NN \cite{zhang2019novel}, FCCA \cite{hua2020fcca}, etc. have been able to achieve high performance on clone detection benchmarks. However, there exist some problems with using CCD models for data inclusion detection. Namely, the high cost of training/re-training/inference of large DL models, and the computational infeasibility of attempting clone detection in a pair-wise manner for all of the codes that exist in a dataset. 
    
    % % \subsection{Detecting ML-Generated Content}\label{subsec:background__copyright_in_ml}
    % % \Foutse{just define the concept of memorization since your approach is built on it...no need to talk about it as a failure to generalize...just explain what it is conceptually so that people understand how that aspect of models can be leveraged to extract training information!!!}
        
    % %     \sout{The memorization issue is a long-standing problem in ML, and in the ML community it is regarded more as a ``failure to generalize'' and therefore a failure to ``learn'' \cite{zhang2021understanding}. As a result, the issue of \textit{derivative work} (work generated by an ML model that highly resembles what was present in its training data) is mostly a subject of discussion outside of the ML community. In contrast, the majority of research in ML is focused on determining whether a particular output was generated by an ML model.} \Foutse{the following is more of related works...it doesn't belong here!!!} The DeepFake Detection Challenge (DFDC) \cite{lyu2020deepfake} was introduced by Meta in order to design ways to detect images that were generated by GenAI tools and statistical testing is used to detect machine-generated text \cite{gehrmann2019gltr, mitchell2023detectgpt}. Another approach for detecting machine-generated content is \textit{watermarking}. Watermarking techniques involve embedding information either in the network itself or in the network's outputs in order to prove that content was generated by the network \cite{boenisch2021systematic}. 
        
    % % \\ \textit{Membership Inference Attacks} (MIA) \cite{shokri2017membership} \Foutse{please define membership attacks conceptually and not in a narrative way like this!!!!} \sout{are proposed as a way to extract information from a model by querying the model on specific elements that the model can have no information on unless it has been present in its dataset. However, research in this area is mainly centered around data privacy and the risks of recovering sensitive data from the model by proposing approaches for both attack and defense. As our work is inspired by such approaches, we will dive deeper into this area in Section \ref{sec:related_wors}.}
    % %     \Foutse{please define the concept of MIA in this section!!!! and don't tell stories about it as you are doing currently!!!}

    % \subsection{Membership Inference Attacks}\label{subsec:background__mia}
    %     Memorization a long-standing problem in ML in which an ML model re-creates instances from its training data instead of generalizing \cite{zhang2021understanding}. By exploiting the memorization problem, Membership Inference Attacks (MIA) \cite{shokri2017membership} have shown to be able to extract information from ML models regarding their training data. Shokri et al. \cite{shokri2017membership} studied how an attacker can identify the presence of a record in a model's training dataset by analyzing the model's output probabilities. Based on Shokri et al.'s work, many approaches have been proposed for both attacks on a model for extracting information about its training dataset and defenses in order to prevent the model from recreating sensitive records \cite{shokri2017membership, jia2019memguard, hu2021ear, hui2021practical}. Carlini et al. \cite{carlini2021extracting} attempted to extract the training data of GPT-2 by initializing the model with a sequence start token and having the model generate tokens until it generates an end-of-sequence token. They generate a large number of sequences in this fashion and remove samples that contain low likelihood. Their approach is based on the idea that samples with high likelihood are generated either because of trivial memorization or repeated sub-strings in their dataset. By doing so, they were able to extract information about individuals' contact information, news pieces, tweets, etc. In another work, Carlini et al. \cite{carlini2022quantifying} study the quantity of memorization in LLMs. They show that by increasing the number of parameters of a model, the amount of memorized data increases as well. Chang et al. \cite{chang2023speak} attempt to probe ChatGPT and GPT-4 by using ``name cloze'' membership inference queries. In their approach, they query ChatGPT/GPT-4 by giving it a context (which in their work are texts extracted from novels), mask the token which contains a \textit{name}, and inspect the output's similarity to the original token. The underlying idea is that without the model seeing the input during its training, the name should be impossible to predict. ``Counterfactual Memorization'' \cite{zhang2021counterfactual} is another approach proposed for studying the memorization issue in LLMs. Here, the changes in a model's predictions are characterized by omitting a particular document during its training. Even though this approach shows promise in studying a model's degree of memorization, it is very computationally expensive. To the best of our knowledge, there exists no approach that inspects \textit{LLMs trained on code} in order to detect data inclusion.

    % \subsection{Detecting ML-Generated Content}\label{subsec:background__copyright_in_ml}
    % \Foutse{just define the concept of memorization since your approach is built on it...no need to talk about it as a failure to generalize...just explain what it is conceptually so that people understand how that aspect of models can be leveraged to extract training information!!!}
        
    %     \sout{The memorization issue is a long-standing problem in ML, and in the ML community it is regarded more as a ``failure to generalize'' and therefore a failure to ``learn'' \cite{zhang2021understanding}. As a result, the issue of \textit{derivative work} (work generated by an ML model that highly resembles what was present in its training data) is mostly a subject of discussion outside of the ML community. In contrast, the majority of research in ML is focused on determining whether a particular output was generated by an ML model.} \Foutse{the following is more of related works...it doesn't belong here!!!} The DeepFake Detection Challenge (DFDC) \cite{lyu2020deepfake} was introduced by Meta in order to design ways to detect images that were generated by GenAI tools and statistical testing is used to detect machine-generated text \cite{gehrmann2019gltr, mitchell2023detectgpt}. Another approach for detecting machine-generated content is \textit{watermarking}. Watermarking techniques involve embedding information either in the network itself or in the network's outputs in order to prove that content was generated by the network \cite{boenisch2021systematic}. BROTHER!!!!!! KEEP AN EYE ON THIS
        
    % \\ \textit{Membership Inference Attacks} (MIA) \cite{shokri2017membership} \Foutse{please define membership attacks conceptually and not in a narrative way like this!!!!} \sout{are proposed as a way to extract information from a model by querying the model on specific elements that the model can have no information on unless it has been present in its dataset. However, research in this area is mainly centered around data privacy and the risks of recovering sensitive data from the model by proposing approaches for both attack and defense. As our work is inspired by such approaches, we will dive deeper into this area in Section \ref{sec:related_wors}.}
    %     \Foutse{please define the concept of MIA in this section!!!! and don't tell stories about it as you are doing currently!!!}

% ##### OLD ALGO 3
        % \begin{algorithm}[htb]
        %     \caption{Comparison}
        %     \scriptsize
        %     \SetKwFunction{Predict}{Predict}
        %     \SetKwFunction{SemanticComparison}{SemanticComparison}
        %     \SetKwComment{Comment}{/* }{ */}
        %     \SetKwFunction{AccumulateResults}{AccumulateResults}
            
        %     \KwIn{ModelPredictions \Comment*[r]{Output of Algorithm \ref{algo:algo_inference}.}}
        %     \KwOut{(VariableHits, FunctionHits, ClassHits, StringHits, CommentHits, DocStringHits)}
            
        %     \tcp{Compare the given model's outputs to the masked element depending on its type (i.e. syntactic/semantic)}
            
        %     \ForEach{$(o_i, i) \in  ModelPredictions$}{
        %         \If{$i$ is a syntactic identifier}{
        %             \eIf{$o_i == i$}{
        %                 store $(1, o_i, i)$ in $ComparisonResults$\;
        %             }{
        %                 store $(0, o_i, i)$ in $ComparisonResults$\;
        %             }
        %         }
                
        %         \If{$i$ is a semantic identifier}{
        %             $SemanticSimilarity \leftarrow \SemanticComparison(o_i, i)$\;
                    
        %             \eIf{$SemanticSimilarity \geq SemanticThreshold$}{
        %                 store $(1, o_i, i)$ in $ComparisonResults$\;
        %             }{
        %                 store $(0, o_i, i)$ in $ComparisonResults$\;
        %             }
        %         }
        %     }
            
        %     \tcp{Accumulate the results of similarity for each script}
        %     \ForEach{$r \in ComparisonResults$}{
        %         \If {$r$ corresponds to a variable name}{
        %             $VariableHits \leftarrow VariableHits + r[0]$\;
        %         }
        %         \If{$r$ corresponds to a function name}{
        %             $FunctionHits \leftarrow FunctionHits + r[0]$\;
        %         }
        %         \If{$r$ corresponds to a class name}{
        %             $ClassHits \leftarrow ClassHits + r[0]$\;
        %         }
        %         \If{$r$ corresponds to a string}{
        %             $StringHits \leftarrow StringHits + r[0]$\;
        %         }
        %         \If{$r$ corresponds to a comment}{
        %             $CommentHits \leftarrow CommentHits + r[0]$\;
        %         }
        %         \If{$r$ corresponds to a docstring}{
        %             $DocStringHits \leftarrow DocStringHits + r[0]$\;
        %         }
        %     }
        
        %     \KwRet{(VariableHits, FunctionHits, ClassHits, StringHits, CommentHits, DocStringHits)}\;
        %     \label{algo:algo_comparison}
        % \end{algorithm}

==> table_sample.tex <==
        \begin{table}
            \resizebox{\textwidth}{!}{
                \centering
                \begin{tabular}{c c r r r r r}
                    \toprule
                    Edit Distance Threshold & Repository Inclusion Criterion & Precision(\%) & Accuracy(\%) & F-score(\%) & Sensitivity(\%) & Specificity (\%)\\
                    \midrule
                        \multirow{3}{*}{\textbf{20}} & Considering only a \textbf{single} positive & 88.07 & 83.87 & \underline{88.57} & 89.08 & \underline{71.6}\\
                        & Considering a threshold of \textbf{0.4} & 76.52 & 75.1 & 84.82 & 95.13 & 20.63\\
                        & Considering a threshold of \textbf{0.6} & 80.46 & 71.26 & 80.31 & 80.15 & 47.08\\
                    \midrule
                        \multirow{3}{*}{\textbf{40}} & Considering only a \textbf{single} positive & 79.57 & 79.11 & 83.39 & 94.49 & 42.91\\
                        & Considering a threshold of \textbf{0.4} & 72.96 & 72.4 & 83.8 & 98.43 & 3.62\\
                        & Considering a threshold of \textbf{0.6} & 75.5 & 73.96 & 84.1 & 94.9 & 18.65\\
                    \midrule
                        \multirow{3}{*}{\textbf{60}} & Considering only a \textbf{single} positive & 78.09 & 77.46 & 85.46 & 94.36 & 37.7\\
                        & Considering a threshold of \textbf{0.4} & 71.28 & 71.23 & 82.95 & \underline{99.19} & 2.92\\
                        & Considering a threshold of \textbf{0.6} & 73.3 & 72.11 & 82.89 & 95.38 & 15.6\\
                    \midrule
                        \multirow{3}{*}{\textbf{70}} & Considering only a \textbf{single} positive & 78.47 & 78.08 & 85.85 & 94.77 & 38.81 \\
                        & Considering a threshold of \textbf{0.4} & 73.3 & 72.83 & 84.17 & 98.83 & 2.11\\
                        & Considering a threshold of \textbf{0.6} & 75.46 & 74.11 & 84.39 & 95.71 & 15.34\\
                    \midrule
                        \multirow{3}{*}{\textbf{80}} & Considering only a \textbf{single} positive & 77.79 & 77.47 & 85.55 & 95.02 & 36.17\\
                        & Considering a threshold of \textbf{0.4} & 71.22 & 70.83 & 82.84 & 99 & 1.47\\
                        & Considering a threshold of \textbf{0.6} & 72.42 & 70.98 & 82.41 & 95.6 & 10.3\\
                    \bottomrule
                \end{tabular}
            }
            \caption{Results of TraWiC's code inclusion detection with different edit distance thresholds}
            \label{table:edit_distance_sensitivity_results_repo_level}
        \end{table}

==> tables_sensitivity.tex <==
\begin{table}
                \resizebox{\textwidth}{!}{
                    \centering
                    \begin{tabular}{c c c r r r r r}
                        \toprule
                        Edit Distance Threshold & Noise Ratio & Repository Inclusion Criterion & Precision(\%) & Accuracy(\%) & F-score(\%) & Sensitivity(\%) & Specificity (\%)\\
                        \midrule
                            \multirow{9}{*}{\textbf{20}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 88 & 83.08 & 88.13 & 88.26 & 70.29\\
                            && Considering a threshold of \textbf{0.4} positive & 79.56 & 76.82 & 86.16 & 93.96 & 20\\
                            && Considering a threshold of \textbf{0.6} positive & 80.73 & 67.54 & 78.22 & 75.86 & 40\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 86.4 & 79.25 & 85.22 & 84.08 & 67.43\\
                            && Considering a threshold of \textbf{0.4} positive & 78.67 & 74.83 & 84.93 & 92.24 & 17.14\\
                            && Considering a threshold of \textbf{0.6} positive & 81.13 & 66.88 & 77.47 & 74.13 & 42.85\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 87.8 & 69.04 & 75.1 & 65.62 & 77.49\\
                            && Considering a threshold of \textbf{0.4} positive & 78.51 & 74.17 & 84.46 & 91.37 & 17.14\\
                            && Considering a threshold of \textbf{0.6} positive & 83.5 & 66.22 & 76.05 & 69.82 & 54.28\\
                        
                        \midrule
                            \multirow{9}{*}{\textbf{60}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 79.44 & 78.51 & 86.18 & 94.17 & 39.85\\
                            && Considering a threshold of \textbf{0.4} positive & 77.85 & 78.14 & 87.54 & 93.1 & 5.71\\
                            && Considering a threshold of \textbf{0.6} positive & 80.57 & 79.47 & 87.84 & 96.55 & 22.85\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 79.29 & 74.89 & 83.23 & 87.59 & 43.54\\
                            && Considering a threshold of \textbf{0.4} positive & 77.85 & 78.14 & 87.54 & 93.1 & 5.71\\
                            && Considering a threshold of \textbf{0.6} positive & 81.02 & 79.47 & 87.74 & 95.68 & 25.71\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 81.81 & 59.73 & 66.37 & 55.82 & 69.37\\
                            && Considering a threshold of \textbf{0.4} positive & 78.37 & 78.8 & 87.87 & 99.1 & 8.57\\
                            && Considering a threshold of \textbf{0.6} positive & 84.83 & 83.89 & 85.34 & 85.34 & 40\\
                                                
                        \midrule
                            \multirow{9}{*}{\textbf{80}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 78.92 & 78.03 & 85.93 & 94.31 & 37.82\\
                            && Considering a threshold of \textbf{0.4} positive & 77.85 & 78.14 & 87.54 & 96.13 & 5.71\\
                            && Considering a threshold of \textbf{0.6} positive & 80.71 & 80.13 & 88.28 & 97.41 & 22.85\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 78.42 & 74.94 & 83.54 & 89.38 & 39.29\\
                            && Considering a threshold of \textbf{0.4} positive & 77.33 & 77.48 & 87.21 & 93.1 & 2.85\\
                            && Considering a threshold of \textbf{0.6} positive & 82.01 & 82.11 & 89.41 & 98.27 & 28.57\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 79.1 & 65.58 & 74.37 & 70.17 & 54.24\\
                            && Considering a threshold of \textbf{0.4} positive & 78.37 & 78.8 & 87.87 & 99.1 & 8.57\\
                            && Considering a threshold of \textbf{0.6} positive & 82.7 & 80.79 & 88.35 & 94.82 & 34.28\\
                        \bottomrule
                    \end{tabular}
                }
                \caption{Results of TraWiC's code inclusion detection with different edit distance thresholds - Syntactic}
                \label{table:noise_sensitivity_results_repo_level}
            \end{table}

            \begin{table}
                \resizebox{\textwidth}{!}{
                    \centering
                    \begin{tabular}{c c c r r r r r}
                        \toprule
                        Edit Distance Threshold & Noise Ratio & Repository Inclusion Criterion & Precision(\%) & Accuracy(\%) & F-score(\%) & Sensitivity(\%) & Specificity (\%)\\
                        \midrule
                            \multirow{9}{*}{\textbf{20}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 87.19 & 82.28 & 87.61 & 88.04 & 68.08\\
                            && Considering a threshold of \textbf{0.4} & 79.56 & 76.82 & 86.16 & 93.96 & 20\\
                            && Considering a threshold of \textbf{0.6} & 84.54 & 73.5 & 82.3 & 80.17 & 51.42\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 86.4 & 79.25 & 85.22 & 84.08 & 67.43\\
                            && Considering a threshold of \textbf{0.4} & 83.82 & 74.89 & 81.97 & 80.19 & 61.8\\
                            && Considering a threshold of \textbf{0.6} & 85.32 & 74.17 & 82.66 & 80.17 & 54.28\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 81.69 & 51.86 & 55.22 & 41.7 & 76.93\\
                            && Considering a threshold of \textbf{0.4} & 80.15 & 75.49 & 85.02 & 90.51 & 25.71\\
                            && Considering a threshold of \textbf{0.6} & 87.17 & 61.58 & 70.1 & 58.62 & 71.42\\
                        
                        \midrule
                            \multirow{9}{*}{\textbf{60}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 79.63 & 78.67 & 86.26 & 94.09 & 40.59\\
                            && Considering a threshold of \textbf{0.4} & 78.37 & 78.8 & 87.87 & 93.1 & 8.57\\
                            && Considering a threshold of \textbf{0.6} & 81.42 & 81.45 & 89.06 & 98.27 & 25.71\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 78.82 & 76.32 & 84.58 & 91.25 & 39.48\\
                            && Considering a threshold of \textbf{0.4} & 78.37 & 78.8 & 87.87 & 93.1 & 8.57\\
                            && Considering a threshold of \textbf{0.6} & 81.15 & 80.13 & 88.18 & 96.55 & 25.71\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 78.78 & 74.3 & 82.89 & 87.44 & 41.88\\
                            && Considering a threshold of \textbf{0.4} & 78.23 & 78.14 & 87.45 & 99.13 & 8.57\\
                            && Considering a threshold of \textbf{0.6} & 80.74 & 78.14 & 86.85 & 93.96 & 25.71\\
                                                
                        \midrule
                            \multirow{9}{*}{\textbf{80}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 79.31 & 78.88 & 86.51 & 95.14 & 38.74\\
                            && Considering a threshold of \textbf{0.4} & 77.70 & 77.48 & 87.12 & 99.13 & 5.71\\
                            && Considering a threshold of \textbf{0.6} & 80.71 & 80.13 & 88.28 & 97.41 & 22.85\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 78.03 & 76.75 & 85.16 & 93.72 & 34.87\\
                            && Considering a threshold of \textbf{0.4} & 77.33 & 77.48 & 87.21 & 93.1 & 2.85\\
                            && Considering a threshold of \textbf{0.6} & 80.71 & 80.13 & 88.28 & 97.41 & 22.85\\
                        \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 78.12 & 75.21 & 83.86 & 90.5 & 37.45\\
                            && Considering a threshold of \textbf{0.4} & 77.85 & 78.14 & 87.54 & 99.1 & 5.71\\
                            && Considering a threshold of \textbf{0.6} & 81.42 & 81.45 & 89.06 & 98.27 & 25.71\\
                        \bottomrule
                    \end{tabular}
                }
                \caption{Results of TraWiC's code inclusion detection with different edit distance thresholds - Semantic}
                \label{table:noise_sensitivity_results_repo_level_sem_level}
            \end{table}

            \begin{table}
                \resizebox{\textwidth}{!}{
                    \centering
                    \begin{tabular}{c c c r r r r r}
                        \toprule
                        Edit Distance Threshold & Noise Ratio & Repository Inclusion Criterion & Precision(\%) & Accuracy(\%) & F-score(\%) & Sensitivity(\%) & Specificity (\%)\\
                        \midrule
                            \multirow{9}{*}{\textbf{20}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 87.16\% & 82.07\% & 87.45\% & 87.74\% & 68.08\%\\
                            && Considering a threshold of \textbf{0.4} & 79.71\% & 77.48\% & 86.61\% & 94.83\% & 20.00\%\\
                            && Considering a threshold of \textbf{0.6} & 83.93\% & 73.51\% & 82.46\% & 81.03\% & 48.57\%\\
                            \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 83.37\% & 73.03\% & 83.19\% & 87.03\% & 51.43\%\\
                            && Considering a threshold of \textbf{0.4} & 79.71\% & 77.48\% & 86.61\% & 94.83\% & 20.00\%\\
                            && Considering a threshold of \textbf{0.6} & 85.45\% & 74.83\% & 83.19\% & 81.03\% & 54.29\%\\
                            \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 85.25\% & 50.96\% & 52.18\% & 37.59\% & 83.95\%\\
                            && Considering a threshold of \textbf{0.4} & 82.11\% & 70.50\% & 84.52\% & 87.03\% & 33.14\%\\
                            && Considering a threshold of \textbf{0.6} & 87.84\% & 60.26\% & 68.42\% & 56.03\% & 74.29\%\\
                        \midrule
                            \multirow{9}{*}{\textbf{60}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 79.10\% & 77.87\% & 85.72\% & 93.65\% & 38.95\%\\
                            && Considering a threshold of \textbf{0.4} & 77.70\% & 77.48\% & 87.16\% & 93.10\% & 3.81\%\\
                            && Considering a threshold of \textbf{0.6} & 81.43\% & 81.46\% & 89.06\% & 98.28\% & 25.71\%\\
                            \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 78.93\% & 73.51\% & 82.15\% & 95.14\% & 2.86\%\\
                            && Considering a threshold of \textbf{0.4} & 77.18\% & 76.82\% & 86.79\% & 99.14\% & 2.86\%\\
                            && Considering a threshold of \textbf{0.6} & 80.60\% & 77.48\% & 86.40\% & 93.10\% & 25.71\%\\
                            \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 81.97\% & 54.10\% & 58.53\% & 45.52\% & 75.28\%\\
                            && Considering a threshold of \textbf{0.4} & 79.17\% & 78.81\% & 87.69\% & 99.13\% & 25.71\%\\
                            && Considering a threshold of \textbf{0.6} & 82.57\% & 70.20\% & 80.00\% & 77.59\% & 45.71\%\\
                        \midrule
                            \multirow{9}{*}{\textbf{80}} & 
                            \multirow{3}{*}{0.1} & Considering only a \textbf{single} positive & 78.34\% & 77.39\% & 85.59\% & 94.32\% & 35.61\%\\
                            && Considering a threshold of \textbf{0.4} & 77.7\% & 77.48\% & 87.12\% & 99.14\% & 5.71\%\\
                            && Considering a threshold of \textbf{0.6} & 82.01\% & 82.12\% & 89.41\% & 98.28\% & 28.57\%\\
                            \cline{2-8} & 
                            \multirow{3}{*}{0.5} & Considering only a \textbf{single} positive & 78.12\% & 74.36\% & 83.15\% & 92.89\% & 28.57\%\\
                            && Considering a threshold of \textbf{0.4} & 77.7\% & 77.48\% & 87.12\% & 99.14\% & 5.71\%\\
                            && Considering a threshold of \textbf{0.6} & 81.29\% & 80.79\% & 87.63\% & 91.41\% & 72.32\%\\
                            \cline{2-8} & 
                            \multirow{3}{*}{0.9} & Considering only a \textbf{single} positive & 82.1\% & 73.81\% & 82.99\% & 83.62\% & 14.29\%\\
                            && Considering a threshold of \textbf{0.4} & 79.17\% & 78.51\% & 87.66\% & 98.28\% & 40.00\%\\
                            && Considering a threshold of \textbf{0.6} & 82.2\% & 82.69\% & 87.69\% & 93.62\% & 44.20\%\\
                        \bottomrule
                    \end{tabular}
                }
                \caption{Results of TraWiC's code inclusion detection with different edit distance thresholds - combined}
                \label{table:noise_sensitivity_results_repo_level_combined}
            \end{table}
